5GC$^2$ache: Improving 5G UPF Performance via Cache Optimization

Last Level Cache (LLC) is a precious and critical resource that impacts the performance of applications running on top of CPUs. In this paper, we reveal the significant impact of LLC on the performance of the 5G user plane function (UPF) when running a cloudified 5G core on general-purposed servers. With extensive measurements showing that the throughput can degrade by over 50\% when the precious LLC resource of UPF is not properly allocated, we identify three categories of performance degradation caused by incorrect LLC usage: DMA leakage problem, hot/cold mbuf problem and cache contention. To address these problems, we introduce the design and implementation of 5GC$^2$ache that monitors the LLC status as well as the throughput performance and dynamically adjusts key parameters of the LLC resource allocation. Our experiments show that 5GC$^2$ache enables a commercial 5G core to increase its throughput to 76.41Gbps, 39.41\% higher than the original performance and 29.55\% higher than the state-of-the-art.

==> tex/case.tex <==
\section{Case Study}
\label{sec:case}

\parabf{Baseline, anonymous
vendor:} 

\parabf{Baseline under \sysname, with parameter optimization:} 

\parabf{Baseline under \sysname, without any modification:} 


==> tex/overview.tex <==
\section{\sysname Overview}
\label{sec:overview}

{
% \setlength{\abovecaptionskip}{-2pt}
% \setlength{\belowcaptionskip}{-14pt}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/overview-v3.pdf}
  % \vspace{-0.2in}
  \caption{\sysname overview.}
  \label{fig:overview}

\end{figure}
}

Figure~\ref{fig:overview} shows an overview of \sysname which has three subsystems. 

\squishlist

\item \textbf{\wm{Alleviating DMA leakage}:} %preventing
This subsystem targets at choosing the correct \wm{number} of RX descriptors to minimize the probability of DMA leakage. The challenge of designing this module is balancing the tradeoff between packet loss rate and DMA leakage. When the number of RX descriptors is \be{small}, we observe a higher packet loss rate and less DMA leakage. When the number is \be{large}, we have the opposite observation. \sysname balances the two and selects the optimal number of RX descriptors that can maximize UPF performance.

\item \textbf{Resolving hot/cold mbuf issues:}
This subsystem chooses the correct size of RX buffer to resolve the hot/cold mbuf issues. When the size of RX buffer is large, we observe severe hot/cold mbuf issues. When the size is small, the UPF throughput degrades because \wm{UPF faces the mbuf shortage issue.} 
% the NIC does not have sufficient memory for storing received packets. 
\sysname balances the two factors and chooses the optimal size of RX buffer that can maximize UPF performance.

\item \textbf{Reducing cache contention:}
This subsystem reduces the cache contention between \wm{DDIO} and CPU core by introducing two mechanisms. First, \sysname configures the DDIO cache and core cache in isolation mode, meaning that the cache resource is not shared between DDIO and CPU core anymore. Second, \sysname dynamically adjusts the size of DDIO cache and core cache to meet the demand of processing traffic with different size of packets.
\squishend
